An Industry Interview Study of Software Signing for Supply Chain Security

Many software products are composed of components integrated from other teams or external parties. Each additional link in a software product's supply chain increases the risk of the injection of malicious behavior. To improve supply chain provenance, many cybersecurity frameworks, standards, and regulations recommend the use of software signing. However, recent surveys and measurement studies have found that the adoption rate and quality of software signatures are low. We lack in-depth industry perspectives on the challenges and practices of software signing. To understand software signing in practice, we interviewed 18 experienced security practitioners across 13 organizations. We study the challenges that affect the effective implementation of software signing in practice. We also provide possible impacts of experienced software supply chain failures, security standards, and regulations on software signing adoption. To summarize our findings: (1) We present a refined model of the software supply chain factory model highlighting practitioner's signing practices; (2) We highlight the different challenges-technical, organizational, and human-that hamper software signing implementation; (3) We report that experts disagree on the importance of signing; and (4) We describe how internal and external events affect the adoption of software signing. Our work describes the considerations for adopting software signing as one aspect of the broader goal of improved software supply chain security.

==> ethics-example.tex <==
\pagebreak

\textit{The call for papers states that an extra page is allotted to discuss ethics considerations and compliance with the open science policy. This page contains that content.}

\section{Ethical Considerations}

This work considers the human and organizational factors governing the adoption of software signing techniques in software engineering work.
To elicit this data, we developed a research protocol, including subject recruitment, interview content, and data processing and analysis.
This protocol was approved by our organization's Institutional Review Board (IRB) prior to the study conduct.
All members of the research team who interacted with subjects or their non-anonymized data have completed our organization's training procedures for handling personally identifiable information.
Data from individual subjects were anonymized following best practices for qualitative data analysis.

Any human-subjects research effort must weigh the risks and benefits for individual research subjects as well as for society.
The primary \textit{risk} for subjects is the hazard to their individual or organizational reputation when describing what might be interpreted as sub-standard cybersecurity practices.
We therefore anonymized subjects by rank and by organization.
A secondary cost for subjects was their time.
Subjects were not coerced to participate, and we offered an incentive of \$100 for their participation.
The primary potential \textit{benefit} for our subjects, their organizations, and the societies in which they operate, is that the resulting data may motivate improvements in the software signing ecosystem, as we discussed in~\cref{sec:Discussion}.
In our judgment, the potential benefit to software cybersecurity far outweighs the risks posed to our subjects and their organizations.

We therefore attest that:
\begin{itemize}
    \item We read the ethics considerations discussions in the conference call for papers, the detailed submissions instructions, and the guidelines for ethics document.
    \item The research team considered the ethics of this research, that the authors believe the research was done ethically, and that the team's next-step plans (\eg after publication) are ethical.
 \end{itemize}

\section{Compliance with Open Science Policy} \label{sec:OpenScience}

We acknowledge that USENIX Security has an open science policy: that authors are expected to openly share their research artifacts by default.
The research artifacts associated with this study are:
\begin{itemize}
    \item Raw transcripts of interviews
    \item Anonymized transcripts of interviews
    \item Interview protocol
    \item Codebook
\end{itemize}

\myparagraph{Things we have shared}
The \textit{interview protocol} is a crucial part of any interview study, since it allows for the critical review of a study design as well as its replication.
Our full interview protocol is included in~\cref{sec:appendix-InterviewProtocol}.
Since it is semi-structured, we include all of the questions asked of all subjects, as well as examples of the follow-up questions we asked.
We also share the \textit{codebook}, with codes, definitions, and example quotes that we coded for each code --- see~\cref{sec:appendix-Codebooks}.

\myparagraph{Things we cannot share}
For subject privacy reasons, and for IRB compliance, we cannot share the raw transcripts.
We are also unwilling to share the anonymized transcripts of the interviews.
Given the high organizational ranks of many of our subjects, and the small size of the subject pool resulting from our recruiting strategy, we believe there is a high risk of de-anonymization even of anonymized transcripts. Therefore, we cannot share the anonymized transcripts.

\raggedbottom
\pagebreak

==> misc/typesetting-old.tex <==
% Pre-condition: Set the ifs: \ifDEBUG, \ifANONYMOUS, \ifSPACEHACK

%%%%%
% Standard packages
%%%%%


%\usepackage[compress]{cite} % numbered ordering of multiple citations, set to compress ranges
\usepackage{amsmath,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{booktabs} % For formal tables \toprule
\usepackage{xspace} % Put an \xspace within numeric macros
\usepackage[normalem]{ulem}
\usepackage{makecell}
\usepackage{tcolorbox}
\usepackage{enumitem}
\usepackage{siunitx}
\usepackage[vskip=1em,font=itshape,leftmargin=2em,rightmargin=2em]{quoting}
\usepackage{svg}
\usepackage{listings}
\usepackage{subfigure}
\usepackage{xcolor}
\usepackage{url}
\def\UrlBreaks{\do\/\do-\do_} % Defining where it is okay to wrap a url to a new line. For bibliography.
%\useunder{\uline}{\ul}{}
% \usepackage{filecontents,lipsum}
% \usepackage[noadjust]{cite}
%%%%%
% Comments and TODOs
%%%%%

\usepackage{soul}
\usepackage{hyperref}
\usepackage{cleveref}

\ifDEBUG
    % Floating comment boxes
    \newcommand{\JD}[1]{\textcolor{blue}{[Jamie: #1]}}
    \newcommand{\Kelechi}[1]{\textcolor{olive}{[Kelechi: #1]}}
    \newcommand{\TRS}[1]{\textcolor{orange}{[Taylor: #1]}}
    \newcommand{\AK}[1]{\textcolor{purple}{[Andy: #1]}}
    \newcommand{\ST}[1]{\textcolor{red}{[Santiago: #1]}}
    \newcommand{\SB}[1]{\textcolor{red}{[Saurabh: #1]}}
    \newcommand{\Eman}[1]{\textcolor{teal}{[Eman: #1]}}
    % Inline comments and WIP phrasing
    \newcommand{\TODO}[1]{\hl{#1}}
    \newcommand{\CHOP}[1]{}
    \newcommand{\placeholder}[1]{\hl{#1}}


    \hypersetup{
        pdfpagemode=UseNone % don't show thumbnails or bookmarks on opening
    }

\else
    \newcommand{\JD}[1]{}
    \newcommand{\Kelechi}[1]{}
    \newcommand{\TRS}[1]{}
    \newcommand{\AK}[1]{}
    \newcommand{\ST}[1]{}
    \newcommand{\SB}[1]{}
    \newcommand{\Eman}[1]{}
    \newcommand{\TODO}[1]{}
    \newcommand{\CHOP}[1]{}
    \newcommand{\placeholder}[1]{#1}
\fi

%%%%%
% Paragraph-level labels
%%%%%

%%%%%
% Space hacking
%%%%%

% To reduce spacing after headings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{titlesec}

% \usepackage[compact]{titlesec}
% \titleformat{\section}
%   {\normalfont\Large\bfseries}{\thesection}{1em}{\MakeUppercase}
%     % The bug in the new version 2.10.1 is not properly starting horizontal mode
%     % http://tex.stackexchange.com/questions/299969/titlesec-loss-of-section-numbering-with-the-new-update-2016-03-15
%     \usepackage{etoolbox}
%     \makeatletter
%     \patchcmd{\ttlh@hang}{\parindent\z@}{\parindent\z@\leavevmode}{}{}
%     \patchcmd{\ttlh@hang}{\noindent}{}{}{}
%     \makeatother

% Make a \paragraph that is inline and emphasized
\newcommand{\myparagraph}[1]{\vspace{0.08cm}\noindent\hspace{0.1cm} \textit{#1:}}

\newcommand{\myminisection}[1]{\vspace{0.1cm} \noindent \textbf{#1.}}

\newcommand{\mysubsubsection}[1]{\subsubsection{\textbf{#1}}}

% \ifSPACEHACK
%     % Titlespacing args: \titlespacing{command}{left spacing}{before spacing}{after spacing}[right]
%     \titlespacing*\subsection{0pt}{2pt plus 1.5pt minus 1.5pt}{1pt plus 1.5pt minus 1.5pt}
%     \titlespacing*\subsubsection{0pt}{2pt plus 1pt minus 1pt}{2pt plus 1.5pt minus 1.5pt}
%     \titlespacing*\paragraph{0pt}{2.5pt plus 1.5pt minus 1.5pt}{2pt plus 1.5pt minus 1.5pt}
%     \setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
%     \setlength{\belowcaptionskip}{2pt plus 1pt minus 1pt}
%     \setlength{\floatsep}{2.0pt plus 2.0pt minus 2.0pt}
%     %\setlength{\textfloatsep}{3.0pt plus 2.0pt minus 4.0pt}
%     %\setlength{\intextsep}{2.0pt plus 2.0pt minus 2.0pt}
% \fi

%%%%%%%%
% Peer review
%%%%%%%%


%%%%%%%%
% Balance references
%%%%%%%%

\usepackage{balance} % Put \balance on the last page
%\usepackage{caption}
%\usepackage[font=normal]{caption}
% \usepackage{subcaption}
%%%%
% Intra-paper references
%%%%

\usepackage{amsmath}
\usepackage{cleveref}


\crefformat{section}{\S#2#1#3}
\crefrangeformat{section}{\S#3#1#4--\S#5#2#6}
\crefname{figure}{Figure}{Figures}
\crefname{appendix}{Appendix}{Appendices}
\crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{listing}{Listing}{Listings}
\crefname{theorem}{Theorem}{Theorems}
\crefname{thm}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{equation}{Eqt.}{Eqts.}
\crefformat{Grammar}{Grammar #1}


%%%%
% Tunable enumerate and itemize
%%%%

\usepackage{enumitem}
\usepackage{booktabs}

%%%%
% Latin
%%%%

\newcommand{\ie}{\textit{i.e.,} }
\newcommand{\eg}{\textit{e.g.,} }
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etals}{\textit{et al.'s}\xspace}
\newcommand{\nb}{\textit{N.B.,} }

\newcommand{\HF}{{Hugging Face}\xspace}
% Please add the following required packages to your document preamble:

\usepackage{enumitem}

%\usepackage{booktabs}
%\usepackage[normalem]{ulem}

% Nice formatting for a list of RQs
\newenvironment{RQList}{
   \setlength{\topsep}{0pt}
   \setlength{\partopsep}{0pt}
   \setlength{\parskip}{0pt}
   \begin{description}[style=unboxed]
   \setlength{\leftmargin}{1in}
   \setlength{\parsep}{0pt}
   \setlength{\parskip}{0pt}
   \setlength{\itemsep}{0pt}
   }
   {\end{description}}
   
\setlength{\abovecaptionskip}{2pt plus 1pt minus 1pt}
\setlength{\belowcaptionskip}{2pt plus 1pt minus 1pt}

\newcommand{\myquote}[1]{\begin{quote}\emph{``#1''}\end{quote}}
\newcommand{\myinlinequote}[1]{\emph{``#1''}}

\newcommand{\SmallLongString}[1]{ {\small \emph{#1}}\xspace}

% ParticipantID, Quote
\newcommand{\ParticipantQuote}[2]{
    \begin{quote}
    \emph{\textbf{#1}: ``#2''} 
    \end{quote}}
    
\DeclareUnicodeCharacter{2060}{\nolinebreak}

